Validating Causal Inference Methods

The fundamental challenge of drawing causal inference is that counterfactual outcomes are not fully observed for any unit. Furthermore, in observational studies, treatment assignment is likely to be confounded. Many statistical methods have emerged for causal inference under unconfoundedness conditions given pre-treatment covariates, including propensity score-based methods, prognostic score-based methods, and doubly robust methods. Unfortunately for applied researchers, there is no `one-size-fits-all' causal method that can perform optimally universally. In practice, causal methods are primarily evaluated quantitatively on handcrafted simulated data. Such data-generative procedures can be of limited value because they are typically stylized models of reality. They are simplified for tractability and lack the complexities of real-world data. For applied researchers, it is critical to understand how well a method performs for the data at hand. Our work introduces a deep generative model-based framework, Credence, to validate causal inference methods. The framework's novelty stems from its ability to generate synthetic data anchored at the empirical distribution for the observed sample, and therefore virtually indistinguishable from the latter. The approach allows the user to specify ground truth for the form and magnitude of causal effects and confounding bias as functions of covariates. Thus simulated data sets are used to evaluate the potential performance of various causal estimation methods when applied to data similar to the observed sample. We demonstrate Credence's ability to accurately assess the relative performance of causal estimation techniques in an extensive simulation study and two real-world data applications from Lalonde and Project STAR studies.

==> background.tex <==
\section{Background}\label{sec:background}
\textbf{Causal inference approaches.} Randomized controlled trials (RCT) or A/B tests are considered the gold-standard approaches for causal inference. In RCTs, the units are randomly assigned to either treated or control groups. Randomization of treatment assignment breaks the association between any potential confounder and selection into treatment. Thus, RCTs anchor the selection bias to \textit{null}. In many situations where performing RCTs are infeasible due to ethical, monetary or time constraints, statistical methods are used to control for confounders and estimate causal effects. Commonly used observational causal inference methods can be divided into three main classes: (1) matching, (2) modeling and (3) weighting approaches. 
\textit{Matching methods}, such as nearest neighbors or propensity score matching, create a subgroup of almost identical units (under a distance metric of choice) from different treatment arms and compare the outcome inside the matched group \cite{Stuart10}. Propensity score matching finds units from different treatment arms with similar probability of selecting into one of the treatment arms \cite{rosenbaum1984reducing}. This is one of the most popular approaches used across domains from epidemiology to social sciences due to its simplicity \cite{imbens2015causal}. More recent advancements in matching methods focus on learning a distance metric for estimating heterogeneous treatment effects \cite{malts,flame}. 
\textit{Modeling methods}, on the other hand, directly try to model the relationship between the covariates and potential outcomes. Modeling approaches such as meta-learners have gained popularity due to advancement in non-parametric methods \cite{metalearners}. Recent work on orthogonal/double machine learning literature focuses on developing methods which infer causal effects using the relationship between the residuals from propensity score and outcome models \cite{chernozhukov2018double}. These models are widely used for applications to high-dimensional, large data contexts with heterogeneous causal effects \cite{athey2019machine}.
\paragraph{Conventional Assumptions. } Consider $X$ to be the set of observed covariates such that where $W \subseteq X$, then the identification of treatment effects for most of the causal inference methods typically depend on few key assumptions:
\begin{enumerate}
    \item Ignorability: $Y_i(z)\perp Z_i | X_i$ 
    \item Stable Unit Treatment Values Assumption (SUTVA):
    \begin{enumerate}
        \item $ Y_i(z) \perp Z_j$
        \item There are no different versions of treatment for each unit
    \end{enumerate}
    \item Positivity: for all $t$ and $x$, $0<P(Z_i=z|X_i=x)<1$
\end{enumerate}


\paragraph{Validating causal methods.}
 Various approaches are proposed in the literature to valid or evaluate the performance of causal methods on specific datasets of interest. These approaches are divided into three main categories: (1) face-validity test, (2) placebo tests, and (3) synthetic data tests. Face-validity tests assess the estimated treatment effect against the expert’s intuition. For instance, if a pharmacologist's expected effect of a malaria medication was a reduction in risk of death, but a causal method’s estimate was contrary to the belief, then this fails the face-validity test. This test clearly is neither sufficient nor necessary - violation does not necessarily indicate that the causal estimation method is biased while agreement with expert’s intuition does not imply that the causal estimation method is accurate. Placebo tests are the most widely used validation approach for causal models \cite{athey2017state} and they come in two varieties: “in-time” and “in-sample” placebo tests. An in-time-placebo test reassigns the treatment to a time period before the actual observed treatment and estimates the treatment effect to generate the distribution of treatment effect under null. In-sample-placebo tests, on the contrary, reassign the treatment to a control unit unaffected by the treatment and use the causal inference method to estimate the effect. These tests are valid only under strong assumptions such as: 
 (a) for in-time placebo tests selection into treatment is assumed to be independent of recent pre-treatment outcome because this might lead to reverse causal-dependency bias,
 (b) for in-sample placebo tests the estimated propensity score for each unit is assumed to be correctly estimated.
 
 
Lastly, for synthetic data tests, the design includes an assumption of a data-generating process with a known distribution. This allows access to the ground truth treatment effects to test the accuracy of causal methods on the designed data generating process. However, as the data generating process is handcrafted, it is unlikely to reflect the same level of complexity as real-world data and it can be designed to favor some methods over others \cite{athey2021using,advani2019mostly,knaus2021machine}. Hence, performance of a method on handcrafted synthetic data does not translate to the performance on real-world data. In Section~\ref{sec:method}, we present a framework to generate synthetic datasets with known treatment effects which have similar distribution properties as the observed dataset of interest.

==> dgp1_ate_true.tex <==
\begin{tabular}{lrr}
\toprule
{} &      mean &     stdev \\
\midrule
NonParametric DML         &  1.274334 &  0.327664 \\
Linear DML                &  1.357951 &  0.298922 \\
Doubly Robust (Linear)    &  1.360807 &  0.303794 \\
Linear T Learner          &  1.359000 &  0.301146 \\
Linear S Learner          &  1.331916 &  0.295129 \\
Linear X Learner          &  1.358347 &  0.301116 \\
NonParametric T Learner   &  1.332980 &  0.287272 \\
NonParametric S Learner   &  1.136796 &  0.272957 \\
NonParametric X Learner   &  1.327336 &  0.278865 \\
Causal BART               &  1.366289 &  0.299657 \\
Causal Forest             &  1.338160 &  0.274242 \\
Propensity Score Matching &  1.420476 &  0.295595 \\
TMLE                      &  1.360765 &  0.301824 \\
\bottomrule
\end{tabular}


==> dgp1_bias_credence.tex <==
\begin{tabular}{lrr}
\toprule
{} &      mean &     stdev \\
\midrule
NonParametric DML         & -0.080040 &  0.310193 \\
Linear DML                &  0.040189 &  0.272152 \\
Doubly Robust (Linear)    &  0.045172 &  0.259434 \\
Linear T Learner          &  0.038570 &  0.266342 \\
Linear S Learner          &  0.011045 &  0.260094 \\
Linear X Learner          &  0.038014 &  0.266304 \\
NonParametric T Learner   &  0.053786 &  0.271855 \\
NonParametric S Learner   & -0.168749 &  0.285372 \\
NonParametric X Learner   &  0.052322 &  0.264542 \\
Causal BART               &  0.061710 &  0.274512 \\
Causal Forest             &  0.028003 &  0.269975 \\
Propensity Score Matching &  0.083010 &  0.286051 \\
TMLE                      &  0.040755 &  0.265415 \\
\bottomrule
\end{tabular}


==> dgp1_bias_true.tex <==
\begin{tabular}{lrr}
\toprule
{} &      mean &     stdev \\
\midrule
NonParametric DML         & -0.035127 &  0.327664 \\
Linear DML                &  0.048490 &  0.298922 \\
Doubly Robust (Linear)    &  0.051346 &  0.303794 \\
Linear T Learner          &  0.049540 &  0.301146 \\
Linear S Learner          &  0.022455 &  0.295129 \\
Linear X Learner          &  0.048886 &  0.301116 \\
NonParametric T Learner   &  0.023519 &  0.287272 \\
NonParametric S Learner   & -0.172665 &  0.272957 \\
NonParametric X Learner   &  0.017875 &  0.278865 \\
Causal BART               &  0.056829 &  0.299657 \\
Causal Forest             &  0.028699 &  0.274242 \\
Propensity Score Matching &  0.111016 &  0.295595 \\
TMLE                      &  0.051305 &  0.301824 \\
\bottomrule
\end{tabular}


==> dgp2_ate_true.tex <==
\begin{tabular}{lrr}
\toprule
{} &      mean &     stdev \\
\midrule
NonParametric DML         &  0.457431 &  0.275530 \\
Linear DML                &  0.446167 &  0.103719 \\
Doubly Robust (Linear)    &  0.559287 &  0.176168 \\
Linear T Learner          &  0.556540 &  0.169663 \\
Linear S Learner          &  0.642249 &  0.153478 \\
Linear X Learner          &  0.579761 &  0.160413 \\
NonParametric T Learner   &  0.704717 &  0.131333 \\
NonParametric S Learner   &  0.173387 &  0.077085 \\
NonParametric X Learner   &  0.424019 &  0.112383 \\
Causal BART               &  0.407128 &  0.128126 \\
Causal Forest             &  0.711616 &  0.108826 \\
Propensity Score Matching &  2.600154 &  0.330318 \\
TMLE                      &  0.532849 &  0.174005 \\
\bottomrule
\end{tabular}


==> dgp2_bias_credence.tex <==
\begin{tabular}{lrr}
\toprule
{} &      mean &     stdev \\
\midrule
NonParametric DML         &  0.094253 &  0.304190 \\
Linear DML                &  0.141997 &  0.086832 \\
Doubly Robust (Linear)    &  0.243161 &  0.158778 \\
Linear T Learner          &  0.221791 &  0.112623 \\
Linear S Learner          &  0.309000 &  0.129677 \\
Linear X Learner          &  0.250363 &  0.116336 \\
NonParametric T Learner   &  0.408379 &  0.099964 \\
NonParametric S Learner   & -0.099444 &  0.053788 \\
NonParametric X Learner   &  0.138827 &  0.080419 \\
Causal BART               &  0.116346 &  0.162403 \\
Causal Forest             &  0.416766 &  0.100564 \\
Propensity Score Matching &  2.403844 &  0.277501 \\
TMLE                      &  0.213875 &  0.128100 \\
\bottomrule
\end{tabular}


==> dgp2_bias_true.tex <==
\begin{tabular}{lrr}
\toprule
{} &      mean &     stdev \\
\midrule
NonParametric DML         &  0.150780 &  0.275530 \\
Linear DML                &  0.139517 &  0.103719 \\
Doubly Robust (Linear)    &  0.252636 &  0.176168 \\
Linear T Learner          &  0.249889 &  0.169663 \\
Linear S Learner          &  0.335598 &  0.153478 \\
Linear X Learner          &  0.273111 &  0.160413 \\
NonParametric T Learner   &  0.398066 &  0.131333 \\
NonParametric S Learner   & -0.133264 &  0.077085 \\
NonParametric X Learner   &  0.117368 &  0.112383 \\
Causal BART               &  0.100477 &  0.128126 \\
Causal Forest             &  0.404966 &  0.108826 \\
Propensity Score Matching &  2.293503 &  0.330318 \\
TMLE                      &  0.226198 &  0.174005 \\
\bottomrule
\end{tabular}


==> lalonde_ate_wrt_exp.tex <==
\begin{tabular}{lrr}
\toprule
{} &          mean &         stdev \\
\midrule
NonParametric DML         &  -6383.971453 &  67682.056362 \\
Linear DML                &  -7626.747423 &   2691.684073 \\
Doubly Robust (Linear)    & -14630.508390 &  10921.226247 \\
Linear T Learner          &  -9843.204483 &   1105.467747 \\
Linear S Learner          &   -504.174425 &    556.673719 \\
Linear X Learner          &  -9727.147974 &   1090.520321 \\
NonParametric T Learner   &  -9139.228607 &   2474.705637 \\
NonParametric S Learner   &  -4072.193251 &   1453.188054 \\
NonParametric X Learner   &  -7994.583716 &   2240.405373 \\
Causal BART               &  -8989.544304 &   1391.843450 \\
Causal Forest             &  -2957.525103 &   1026.576502 \\
Propensity Score Matching & -18369.045855 &    865.687243 \\
TMLE                      & -13683.016420 &   1057.882950 \\
\bottomrule
\end{tabular}


==> lalonde_bias_credence.tex <==
\begin{tabular}{lrr}
\toprule
{} &      mean &     stdev \\
\midrule
NonParametric DML         & -0.081514 &  0.209958 \\
Linear DML                & -0.029173 &  0.009904 \\
Doubly Robust (Linear)    & -0.005748 &  0.006498 \\
Linear T Learner          & -0.084196 &  0.010660 \\
Linear S Learner          & -0.003928 &  0.004550 \\
Linear X Learner          & -0.061873 &  0.012586 \\
NonParametric T Learner   & -0.073116 &  0.016059 \\
NonParametric S Learner   & -0.025405 &  0.009419 \\
NonParametric X Learner   & -0.056088 &  0.016048 \\
Causal BART               & -0.074526 &  0.016126 \\
Causal Forest             & -0.022507 &  0.008332 \\
Propensity Score Matching & -0.151962 &  0.007763 \\
TMLE                      & -0.111624 &  0.008831 \\
\bottomrule
\end{tabular}


==> lalonde_bias_wrt_exp.tex <==
\begin{tabular}{lrr}
\toprule
{} &          mean &         stdev \\
\midrule
NonParametric DML         &  -7270.277117 &  67682.056362 \\
Linear DML                &  -8513.053087 &   2691.684073 \\
Doubly Robust (Linear)    & -15516.814054 &  10921.226247 \\
Linear T Learner          & -10729.510147 &   1105.467747 \\
Linear S Learner          &  -1390.480089 &    556.673719 \\
Linear X Learner          & -10613.453638 &   1090.520321 \\
NonParametric T Learner   & -10025.534271 &   2474.705637 \\
NonParametric S Learner   &  -4958.498915 &   1453.188054 \\
NonParametric X Learner   &  -8880.889380 &   2240.405373 \\
Causal BART               &  -9875.849968 &   1391.843450 \\
Causal Forest             &  -3843.830767 &   1026.576502 \\
Propensity Score Matching & -19255.351519 &    865.687243 \\
TMLE                      & -14569.322084 &   1057.882950 \\
\bottomrule
\end{tabular}


==> star_ate_wrt_exp.tex <==
\begin{tabular}{lrr}
\toprule
{} &       mean &       stdev \\
\midrule
NonParametric DML         &  92.935602 &  538.263897 \\
Linear DML                &  21.285413 &    6.052786 \\
Doubly Robust (Linear)    &  20.397505 &    6.410145 \\
Linear T Learner          &  21.738517 &    5.877514 \\
Linear S Learner          &  19.435944 &    6.901133 \\
Linear X Learner          &  21.944491 &    6.121922 \\
NonParametric T Learner   &  24.217762 &    6.702451 \\
NonParametric S Learner   &  19.863004 &    6.434064 \\
NonParametric X Learner   &  23.742269 &    6.891018 \\
Causal BART               &  21.224332 &    5.927698 \\
Causal Forest             &  20.817551 &    5.670172 \\
Propensity Score Matching &  29.431149 &    7.226389 \\
TMLE                      &  23.428819 &    6.586380 \\
\bottomrule
\end{tabular}


==> star_bias_credence.tex <==
\begin{tabular}{lrr}
\toprule
{} &      mean &     stdev \\
\midrule
NonParametric DML         &  0.048795 &  0.008895 \\
Linear DML                &  0.018120 &  0.003472 \\
Doubly Robust (Linear)    &  0.059583 &  0.059835 \\
Linear T Learner          &  0.017263 &  0.003127 \\
Linear S Learner          &  0.017389 &  0.003205 \\
Linear X Learner          &  0.017461 &  0.003120 \\
NonParametric T Learner   &  0.031087 &  0.004524 \\
NonParametric S Learner   &  0.012644 &  0.003838 \\
NonParametric X Learner   &  0.028505 &  0.004966 \\
Causal BART               &  0.015821 &  0.003200 \\
Causal Forest             &  0.041218 &  0.004633 \\
Propensity Score Matching &  0.034142 &  0.003632 \\
TMLE                      & -0.005222 &  0.016977 \\
\bottomrule
\end{tabular}


==> star_bias_wrt_exp.tex <==
\begin{tabular}{lrr}
\toprule
{} &       mean &       stdev \\
\midrule
NonParametric DML         &  85.694352 &  538.263897 \\
Linear DML                &  14.044163 &    6.052786 \\
Doubly Robust (Linear)    &  13.156254 &    6.410145 \\
Linear T Learner          &  14.497267 &    5.877514 \\
Linear S Learner          &  12.194693 &    6.901133 \\
Linear X Learner          &  14.703241 &    6.121922 \\
NonParametric T Learner   &  16.976512 &    6.702451 \\
NonParametric S Learner   &  12.621754 &    6.434064 \\
NonParametric X Learner   &  16.501019 &    6.891018 \\
Causal BART               &  13.983081 &    5.927698 \\
Causal Forest             &  13.576301 &    5.670172 \\
Propensity Score Matching &  22.189898 &    7.226389 \\
TMLE                      &  16.187568 &    6.586380 \\
\bottomrule
\end{tabular}

